Exponential Convergence of $hp$-Time-Stepping in Space-Time Discretizations of Parabolic PDEs

For linear parabolic initial-boundary value problems with self-adjoint, time-homogeneous elliptic spatial operator in divergence form with Lipschitz-continuous coefficients, and for incompatible, time-analytic forcing term in polygonal/polyhedral domains $D$, we prove time-analyticity of solutions. Temporal analyticity is quantified in terms of weighted, analytic function classes, for data with finite, low spatial regularity and without boundary compatibility. Leveraging this result, we prove exponential convergence of a conforming, semi-discrete $hp$-time-stepping approach. We combine this semi-discretization in time with first-order, so-called "$h$-version" Lagrangian Finite Elements with corner-refinements in space into a tensor-product, conforming discretization of a space-time formulation. We prove that, under appropriate corner- and corner-edge mesh-refinement of $D$, error vs. number of degrees of freedom in space-time behaves essentially (up to logarithmic terms), to what standard FEM provide for one elliptic boundary value problem solve in $D$. We focus on two-dimensional spatial domains and comment on the one- and the three-dimensional case.

==> Numerics/2dPoisson/gradedNVBmu06/poissonTriTikzL2.tex <==
        10   0.0699573559717388
        43   0.0463728796745329
       180   0.0153112187020111
       773   0.0039247804204576
      3197   0.0009955131290078
     12991   0.0002558375550584
     52408   0.0000638991565699
    210596   0.0000162198310079
    844244   0.0000040788753927
   3380799   0.0000010257100964
  13530820   0.0000002583168206


==> Numerics/2dPoisson/uniform/poissonTriTikzL2.tex <==
         5   0.1835689461369527
        33   0.0698237800627983
       161   0.0232088282605728
       705   0.0068475292273653
      2945   0.0020430974005071
     12033   0.0006580550992058
     48641   0.0002249112362954
    195585   0.0000819806765157
    784385   0.0000309377334218
   3141633   0.0000119708593604
  12574721   0.0000046766038282


==> Numerics/2du2/hgradedNVBmu06/heatHilbertTriCylTikzH12.tex <==
        40   0.0409409852062445
       344   0.0246705057255904
      2880   0.0090165349628482
     24736   0.0029536970012675
    204608   0.0010182934201951
   1662848   0.0003613694232758
  13416448   0.0001273417828937
 107825152   0.0000453130291202
 864505856   0.0000160638573928


==> Numerics/2du2/huniform/heatHilbertTriCylTikzH12.tex <==
        20   0.0855522861522609
       264   0.0341034032844908
      2576   0.0121377447433463
     22560   0.0041285041185192
    188480   0.0014975965003460
   1540224   0.0005859718785555
  12452096   0.0002397992897407
 100139520   0.0001019241778958
 803210240   0.0000441844906997


==> Numerics/2du2/pgradedNVBmu06/heatHilbertTriCylTikzH12.tex <==
        40   0.0409409852062445
       172   0.0321356993789573
      1440   0.0077056747182743
      9276   0.0017855956684015
     51152   0.0004478457718757
    207856   0.0001151654109604
   1048160   0.0000286914975894
   5054304   0.0000072715871953
  20261856   0.0000018293148744
  94662372   0.0000004596964699


==> Numerics/2du2/puniform/heatHilbertTriCylTikzH12.tex <==
        20   0.0855522861522609
       132   0.0402104057549505
      1288   0.0110498777516473
      8460   0.0030781093514853
     35340   0.0009388440336019
    192528   0.0002917525563651
    972820   0.0000993815711701
   4694040   0.0000361575153092
  18825240   0.0000136390445586
  87965724   0.0000052752736413


==> Numerics/2du3/hgradedNVBmu06/heatHilbertTriCylTikzH12.tex <==
        40   0.0940085438462637
       344   0.0634635439018920
      2880   0.0330577199910305
     24736   0.0165270949172088
    204608   0.0090092804838865
   1662848   0.0053774576987615
  13416448   0.0033912723337871
 107825152   0.0021975854999706
 864505856   0.0014391734256553


==> Numerics/2du3/hpgradedNVBmu06/heatHilbertTriCylTikzH12.tex <==
       200   0.0541482950058803
      1892   0.0359999453380334
     13860   0.0143851936778685
     91987   0.0054122418398553
    543490   0.0020958503147924
   2987930   0.0008206663089518
  15669992   0.0003167101786014
  79394692   0.0001230470023638
 417900780   0.0000461582215051


==> Numerics/2du3/hpuniform/heatHilbertTriCylTikzH12.tex <==
        45   0.1249608618905404
      1155   0.0503281447871460
     12397   0.0185827727238351
     83895   0.0072689371175188
    500650   0.0030138776110593
   2767590   0.0013158005342629
  14543659   0.0005931290593205
  73735545   0.0002760262349386
 363954640   0.0001308532270817


==> Numerics/2du3/hpuniform/heatHilbertTriCylTikzH12_alt.tex <==
        35   0.0935445381330398
      1419   0.0398415173371675
     14651   0.0154219165534190
    110685   0.0067692370251255
    709745   0.0029736875106755
   4127319   0.0013790991549118
  22520783   0.0006530894388531
 117546585   0.0003142975984135
 593779445   0.0001537761671214


==> Numerics/2du3/huniform/heatHilbertTriCylTikzH12.tex <==
        20   0.1108295385173504
       264   0.0639422097809956
      2576   0.0316801544285231
     22560   0.0171160280000298
    188480   0.0096712064374581
   1540224   0.0058491471582257
  12452096   0.0036592191799713
 100139520   0.0023367942400940
 803210240   0.0015085219528781

